Time-fractional Moore-Gibson-Thompson equations

In this paper, we consider several time-fractional generalizations of the Jordan-Moore-Gibson-Thompson (JMGT) equations in nonlinear acoustics as well as their linear Moore-Gibson-Thompson (MGT) versions. Following the procedure described in Jordan (2014), these time-fractional acoustic equations are derived from four fractional versions of the Maxwell-Cattaneo law in Compte and Metzler (1997). Additionally to providing well-posedness results for each of them, we also study the respective limits as the fractional order tends to one, leading to the classical third order in time (J)MGT equation.

==> FixedPoint.tex <==
\section{Well-posedness of the fractional model} \label{Sec:FixedPoint}


==> Introduction.tex <==
\section{Introduction} \label{Sec:Introduction}
\begin{equation} \label{Eq:FracMGT}
\begin{aligned}
\tau^\alpha D_t^{\alpha}\psi_{tt}+(1- k\psi_t)\psi_{tt}-c^2 \D \psi-\tau^\alpha c^2 D_t^\alpha \Delta \psi -\delta D_t^{1-\alpha} \Delta \psi_t= k(|\nabla \psi|^2)_t
\end{aligned}
\end{equation}

==> Limit.tex <==
\section{The limit as $\alpha \rightarrow 1$}  \label{Sec:Limit}

